MIMEx: Intrinsic Rewards from Masked Input Modeling

Exploring in environments with high-dimensional observations is hard. One promising approach for exploration is to use intrinsic rewards, which often boils down to estimating "novelty" of states, transitions, or trajectories with deep networks. Prior works have shown that conditional prediction objectives such as masked autoencoding can be seen as stochastic estimation of pseudo-likelihood. We show how this perspective naturally leads to a unified view on existing intrinsic reward approaches: they are special cases of conditional prediction, where the estimation of novelty can be seen as pseudo-likelihood estimation with different mask distributions. From this view, we propose a general framework for deriving intrinsic rewards -- Masked Input Modeling for Exploration (MIMEx) -- where the mask distribution can be flexibly tuned to control the difficulty of the underlying conditional prediction task. We demonstrate that MIMEx can achieve superior results when compared against competitive baselines on a suite of challenging sparse-reward visuomotor tasks.

==> figures/ablation.tex <==
%\begin{figure*}[t!]
% \begin{center}
% \includegraphics[width=0.8\textwidth]{images/seq_length.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\textbf{Effect of varying exploration sequence length.} \textit{ln} refers to exploration with sequence length of $n$ for $n = 2, 3, 4, 5, 6$.}
% \label{fig:ablation}
% \vspace{-10pt}
% \end{figure*}

% \begin{figure*}[t!]
% \begin{center}
% \includegraphics[width=0.8\textwidth]{images/variance_reduction.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\textbf{Effect of varying number of random masks used to calculate intrinsic reward.} \textit{nm1} is masking once and \textit{nm5} is masking 5 times and taking the average.}
% \label{fig:ablation}
% \vspace{-10pt}
% \end{figure*}

% \begin{figure*}[t!]
% \begin{center}
% \includegraphics[width=0.8\textwidth]{images/scale.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\textbf{Effect of scaling masked autoencoder decoder.} The \textit{larger} model uses a decoder that doubles in depth, number of output heads, and embedding dimensions compared with those of the \textit{smaller} model.}
% \label{fig:ablation}
% \vspace{-10pt}
% \end{figure*}

==> figures/mask_ratio.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{images/mr.pdf}
    \end{center}
    \vspace{-10pt}
    \caption{\textbf{Varying mask ratio.} Results from masking out 20\%, 50\%, and 70\% during the random masking step of MIMEx.}
    \label{fig:mr}
    % \vspace{-10pt}
\end{wrapfigure}

==> figures/mask_type.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{images/mt.pdf}
    \end{center}
    \vspace{-10pt}
    \caption{\textbf{Varying mask type and ratio.} Results from (1) masking only on the time dimension with a mask ratio of 70\% (\textit{70\%}) and (2) masking on the feature dimension with mask ratios of 80\%, 90\%, and 95\% (\textit{80\%(a)}, \textit{90\%(a)}, \textit{95\%(a)}).}
    \label{fig:mt}
    \vspace{-14pt}
\end{wrapfigure}

==> figures/scale.tex <==
\begin{figure}
\centering
    % \includegraphics[width=\columnwidth]{images/scale8x8.pdf}
    % \includegraphics[width=\columnwidth]{images/scale6x8.pdf}
    \includegraphics[width=.5\linewidth]{images/scale.pdf}
    \vspace{-8pt}
    \caption{\textbf{Scaling MIMEx decoder.} Compared with the \textit{smaller} model, the \textit{larger} model uses a decoder that doubles in depth, number of output heads, and embedding dimensions.}
    \label{fig:scale}
    \vspace{-10pt}
\end{figure}


==> figures/seq_length.tex <==
\begin{wrapfigure}{r}{0.55\textwidth}
\begin{center}
% \includegraphics[width=\columnwidth]{images/seq_length8x8.pdf}
\includegraphics[width=\linewidth]{images/seq_length.pdf}
\end{center}
\vspace{-10pt}
\caption{\textbf{Varying exploration sequence length.} l\textit{n} refers to exploration with sequence length of $n$ for $n = 2, 3, 4, 5, 6$.}
\label{fig:seq}
\vspace{-10pt}
\end{wrapfigure}

==> figures/seq_var.tex <==
\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/seq_length.pdf}
  
  \vspace{-8pt}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/variance_reduction.pdf}
  \label{fig:var}
  \vspace{-8pt}
\end{minipage}
\label{fig:seq-var}
\vspace{-10pt}
\caption{\textbf{(left) Varying exploration sequence length.} l\textit{n} refers to exploration with sequence length of $n$ for $n = 2, 3, 4, 5, 6$. \textbf{(right) Varying number of times of masking for intrinsic reward calculation.} \textit{nm1} is masking once, and \textit{nm5} is masking 5 times followed by taking the average of all prediction errors.}
\end{figure}

==> figures/variance_reduction.tex <==
\begin{wrapfigure}{rr r}{0.55\textwidth}
\begin{center}
% \includegraphics[width=\columnwidth]{images/variance_reduction8x8.pdf}
\includegraphics[width=\linewidth]{images/variance_reduction.pdf}
\end{center}
\vspace{-10pt}
\caption{\textbf{Varying number of times of masking for intrinsic reward calculation.} \textit{nm1} is masking once, and \textit{nm5} is masking 5 times followed by taking the average of all prediction errors.}
\label{fig:var}
\vspace{-10pt}
\end{wrapfigure}

==> tables/model.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{0.3\columnwidth}{!}{%
    \begin{tabular}{c|c}
        \hline
         Config  & Value \\
         \hline
         
         encoder embedding dim    &  128         \\
         no. of encoder heads    &  4         \\
         encoder depth    &  4         \\

         decoder embedding dim    &  64         \\
         no. of decoder heads    &  2         \\
         decoder depth    &  1         \\
         \hline
    \end{tabular}
    }\vspace{1pt}%
    \caption{Model implementation details.}
    \label{tbl:model}
\end{table}

==> tables/sparse.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
        \hline
         Task  & Example Steps to Sparsify Rewards \\
         \hline
         
         \textit{FrankaCabinet}     & 1. Remove ``distance to handle'' term          \\
                                     & 2. Remove ``distance to goal'' term         \\
         \hline

         \textit{KukaCabinet}     & 1. Remove ``finger / thumb distance to handle'' terms          \\
                                & 2. Remove ``distance to goal'' term        \\
         \hline
         
         \textit{FrankaPick}     & 1. Remove ``distance to object'' term          \\
                                     & 2. Remove ``distance to goal'' term         \\
         \hline

         \textit{KukaPick}      & 1. Remove ``finger / thumb distance to object'' terms          \\
                                & 2. Remove ``distance to goal'' term        \\
         \hline
         
         \textit{FrankaMove}     & 1. Remove ``distance to object'' term          \\
                                     & 2. Remove ``distance to goal'' term         \\
         \hline

         \textit{KukaMove}     & 1. Remove ``finger / thumb distance to object'' terms          \\
                                & 2. Remove ``distance to goal'' term        \\
         \hline
    \end{tabular}
    }\vspace{1pt}%
    \caption{A sample curriculum to gradually increasing exploration difficulty for each task in PixMC-Sparse.}
    \label{tbl:sparse}
\end{table}

==> tables/sparsify.tex <==
\begin{table}[H]
    \centering
    \small
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
        \hline
         Task  & Removed Dense Reward Terms \\
         \hline
         
         \textit{FrankaReach}     & distance to goal         \\ 
         \hline

         \textit{KukaReach}     & distance to goal           \\
         \hline
         
         \textit{FrankaCabinet}     & distance to handle          \\
         \hline
         
         % \textit{KukaCabinet}     & finger distance to handle          \\
         %                          & thumb distance to handle          \\
         \textit{KukaCabinet}     & finger distance to handle, thumb distance to handle          \\
         \hline
         
         \textit{FrankaPick}     & distance to object          \\
         \hline

         % \textit{KukaPick}     & finger distance to object          \\
         %                       & thumb distance to object          \\
         \textit{KukaPick}     & finger distance to object, thumb distance to object          \\
         \hline
         
         \textit{FrankaMove}     & distance to object          \\
         \hline

         % \textit{KukaMove}     & finger distance to object         \\
         %                      & thumb distance to object          \\
         \textit{KukaMove}     & finger distance to object, thumb distance to object          \\
         \hline
    \end{tabular}
    }\vspace{1pt}%
    \caption{We define PixMC-Sparse tasks by removing reward terms from the reward functions of PixMC tasks. In the table, we show details of how each task reward function is modified.}
    \label{tbl:sparsify}
\end{table}
